GCAN: Graph-aware Co-Attention Networks for Explainable Fake News Detection on Social Media

This paper solves the fake news detection problem under a more realistic scenario on social media. Given the source short-text tweet and the corresponding sequence of retweet users without text comments, we aim at predicting whether the source tweet is fake or not, and generating explanation by highlighting the evidences on suspicious retweeters and the words they concern. We develop a novel neural network-based model, Graph-aware Co-Attention Networks (GCAN), to achieve the goal. Extensive experiments conducted on real tweet datasets exhibit that GCAN can significantly outperform state-of-the-art methods by 16% in accuracy on average. In addition, the case studies also show that GCAN can produce reasonable explanations.

==> mybib.tex <==
@inproceedings{content1,
 author = {Castillo, Carlos and Mendoza, Marcelo and Poblete, Barbara},
 title = {Information Credibility on Twitter},
 booktitle = {Proceedings of the 20th International Conference on World Wide Web},
 series = {WWW '11},
 year = {2011},
 pages = {675--684},
} 


@inproceedings{Ma:2015:DRU:2806416.2806607,
 author = {Ma, Jing and Gao, Wei and Wei, Zhongyu and Lu, Yueming and Wong, Kam-Fai},
 title = {Detect Rumors Using Time Series of Social Context Information on Microblogging Websites},
 booktitle = {Proceedings of the 24th ACM International on Conference on Information and Knowledge Management},
 series = {CIKM '15},
 year = {2015},
 isbn = {978-1-4503-3794-6},
 location = {Melbourne, Australia},
 pages = {1751--1754},
 numpages = {4},
 url = {http://doi.acm.org/10.1145/2806416.2806607},
 doi = {10.1145/2806416.2806607},
 acmid = {2806607},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {rumor detection, social context, temporal, time series},
} 


@article{30c0de09011b4b0c91704bfe29142828,
title = "Detecting rumors from microblogs with recurrent neural networks",
abstract = "Microblogging platforms are an ideal place for spreading rumors and automatically debunking rumors is a crucial problem. To detect rumors, existing approaches have relied on hand-crafted features for employing machine learning algorithms that require daunting manual effort. Upon facing a dubious claim, people dispute its truthfulness by posting various cues over time, which generates long-distance dependencies of evidence. This paper presents a novel method that learns continuous representations of microblog events for identifying rumors. The proposed model is based on recurrent neural networks (RNN) for learning the hidden representations that capture the variation of contextual information of relevant posts over time. Experimental results on datasets from two real-world microblog platforms demonstrate that (1) the RNN method outperforms state-of-the-art rumor detection models that use hand-crafted features; (2) performance of the RNN-based algorithm is further improved via sophisticated recurrent units and extra hidden layers; (3) RNN-based method detects rumors more quickly and accurately than existing techniques, including the leading online rumor debunking services.",
author = "Jing Ma and Wei Gao and Prasenjit Mitra and Sejeong Kwon and Jansen, {Bernard J.} and Wong, {Kam Fai} and Meeyoung Cha",
year = "2016",
month = "1",
day = "1",
language = "English (US)",
volume = "2016-January",
pages = "3818--3824",
journal = "IJCAI International Joint Conference on Artificial Intelligence",
issn = "1045-0823",
}


@article{10.1371/journal.pone.0168344,
    author = {Kwon, Sejeong AND Cha, Meeyoung AND Jung, Kyomin},
    journal = {PLOS ONE},
    publisher = {Public Library of Science},
    title = {Rumor Detection over Varying Time Windows},
    year = {2017},
    month = {01},
    volume = {12},
    url = {https://doi.org/10.1371/journal.pone.0168344},
    pages = {1-19},
    abstract = {This study determines the major difference between rumors and non-rumors and explores rumor classification performance levels over varying time windows—from the first three days to nearly two months. A comprehensive set of user, structural, linguistic, and temporal features was examined and their relative strength was compared from near-complete date of Twitter. Our contribution is at providing deep insight into the cumulative spreading patterns of rumors over time as well as at tracking the precise changes in predictive powers across rumor features. Statistical analysis finds that structural and temporal features distinguish rumors from non-rumors over a long-term window, yet they are not available during the initial propagation phase. In contrast, user and linguistic features are readily available and act as a good indicator during the initial propagation phase. Based on these findings, we suggest a new rumor classification algorithm that achieves competitive accuracy over both short and long time windows. These findings provide new insights for explaining rumor mechanism theories and for identifying features of early rumor detection.},
    number = {1},
    doi = {10.1371/journal.pone.0168344}
}

@paper{AAAI1816826,
	author = {Yang Liu and Yi-Fang Wu},
	title = {Early Detection of Fake News on Social Media Through Propagation Path Classification with Recurrent and Convolutional Networks},
	conference = {AAAI Conference on Artificial Intelligence},
	year = {2018},
	url = {https://www.aaai.org/ocs/index.php/AAAI/AAAI18/paper/view/16826/15707}
}

@inproceedings{Shu:2019:DEF:3292500.3330935,
 author = {Shu, Kai and Cui, Limeng and Wang, Suhang and Lee, Dongwon and Liu, Huan},
 title = {dEFEND: Explainable Fake News Detection},
 booktitle = {Proceedings of the 25th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
 series = {KDD '19},
 year = {2019},
 isbn = {978-1-4503-6201-6},
 location = {Anchorage, AK, USA},
 pages = {395--405},
 numpages = {11},
 url = {http://doi.acm.org/10.1145/3292500.3330935},
 doi = {10.1145/3292500.3330935},
 acmid = {3330935},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {explainable machine learning, fake news, social network},
} 


@article{article,
author = {Kingma, Diederik and Ba, Jimmy},
year = {2014},
month = {12},
pages = {},
title = {Adam: A Method for Stochastic Optimization},
journal = {International Conference on Learning Representations}
}


@inproceedings{2c16b6ad1569495fac0bd5e212852b9d,
title = "Detect rumors in microblog posts using propagation structure via kernel learning",
abstract = "How fake news goes viral via social media? How does its propagation pattern differ from real stories? In this paper, we attempt to address the problem of identifying rumors, i.e., fake information, out of microblog posts based on their propagation structure. We firstly model microblog posts diffusion with propagation trees, which provide valuable clues on how an original message is transmitted and developed over time. We then propose a kernel-based method called Propagation Tree Kernel, which captures high-order patterns differentiating different types of rumors by evaluating the similarities between their propagation tree structures. Experimental results on two real-world datasets demonstrate that the proposed kernel-based approach can detect rumors more quickly and accurately than state-ofthe-art rumor detection models.",
author = "Jing Ma and Wei Gao and Wong, {Kam Fai}",
year = "2017",
month = "1",
day = "1",
doi = "10.18653/v1/P17-1066",
language = "English",
volume = "1",
pages = "708--717",
booktitle = "ACL 2017 - 55th Annual Meeting of the Association for Computational Linguistics, Proceedings of the Conference (Long Papers)",
publisher = "Association for Computational Linguistics (ACL)",
}


@misc{chung2014empirical,
    title={Empirical Evaluation of Gated Recurrent Neural Networks on Sequence Modeling},
    author={Junyoung Chung and Caglar Gulcehre and KyungHyun Cho and Yoshua Bengio},
    year={2014},
    eprint={1412.3555},
    archivePrefix={arXiv},
    primaryClass={cs.NE}
}


@inproceedings{Castillo:2011:ICT:1963405.1963500,
 author = {Castillo, Carlos and Mendoza, Marcelo and Poblete, Barbara},
 title = {Information Credibility on Twitter},
 booktitle = {Proceedings of the 20th International Conference on World Wide Web},
 series = {WWW '11},
 year = {2011},
 isbn = {978-1-4503-0632-4},
 location = {Hyderabad, India},
 pages = {675--684},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1963405.1963500},
 doi = {10.1145/1963405.1963500},
 acmid = {1963500},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {social media analytics, social media credibility, twitter},
} 

@inproceedings{potthast-etal-2018-stylometric,
    title = "A Stylometric Inquiry into Hyperpartisan and Fake News",
    author = "Potthast, Martin  and
      Kiesel, Johannes  and
      Reinartz, Kevin  and
      Bevendorff, Janek  and
      Stein, Benno",
    booktitle = "Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = jul,
    year = "2018",
    address = "Melbourne, Australia",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P18-1022",
    doi = "10.18653/v1/P18-1022",
    pages = "231--240",
    abstract = "We report on a comparative style analysis of hyperpartisan (extremely one-sided) news and fake news. A corpus of 1,627 articles from 9 political publishers, three each from the mainstream, the hyperpartisan left, and the hyperpartisan right, have been fact-checked by professional journalists at BuzzFeed: 97{\%} of the 299 fake news articles identified are also hyperpartisan. We show how a style analysis can distinguish hyperpartisan news from the mainstream (F1 = 0.78), and satire from both (F1 = 0.81). But stylometry is no silver bullet as style-based fake news detection does not work (F1 = 0.46). We further reveal that left-wing and right-wing news share significantly more stylistic similarities than either does with the mainstream. This result is robust: it has been confirmed by three different modeling approaches, one of which employs Unmasking in a novel way. Applications of our results include partisanship detection and pre-screening for semi-automatic fake news detection.",
}


@article{DBLP:journals/corr/abs-1903-01728,
  author    = {Chuan Guo and
               Juan Cao and
               Xueyao Zhang and
               Kai Shu and
               Miao Yu},
  title     = {Exploiting Emotions for Fake News Detection on Social Media},
  journal   = {CoRR},
  volume    = {abs/1903.01728},
  year      = {2019},
  url       = {http://arxiv.org/abs/1903.01728},
  archivePrefix = {arXiv},
  eprint    = {1903.01728},
  timestamp = {Sat, 30 Mar 2019 19:27:21 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1903-01728},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{Popat:2017:ACC:3041021.3053379,
 author = {Popat, Kashyap},
 title = {Assessing the Credibility of Claims on the Web},
 booktitle = {Proceedings of the 26th International Conference on World Wide Web Companion},
 series = {WWW '17 Companion},
 year = {2017},
 isbn = {978-1-4503-4914-7},
 location = {Perth, Australia},
 pages = {735--739},
 numpages = {5},
 url = {https://doi.org/10.1145/3041021.3053379},
 doi = {10.1145/3041021.3053379},
 acmid = {3053379},
 publisher = {International World Wide Web Conferences Steering Committee},
 address = {Republic and Canton of Geneva, Switzerland},
 keywords = {credibility analysis, rumor detection, text analytics},
} 

@inproceedings{Zhao:2015:EME:2736277.2741637,
 author = {Zhao, Zhe and Resnick, Paul and Mei, Qiaozhu},
 title = {Enquiring Minds: Early Detection of Rumors in Social Media from Enquiry Posts},
 booktitle = {Proceedings of the 24th International Conference on World Wide Web},
 series = {WWW '15},
 year = {2015},
 isbn = {978-1-4503-3469-3},
 location = {Florence, Italy},
 pages = {1395--1405},
 numpages = {11},
 url = {https://doi.org/10.1145/2736277.2741637},
 doi = {10.1145/2736277.2741637},
 acmid = {2741637},
 publisher = {International World Wide Web Conferences Steering Committee},
 address = {Republic and Canton of Geneva, Switzerland},
 keywords = {enquiry tweets, rumor detection, social media},
} 


@article{30c0de09011b4b0c91704bfe29142828,
title = "Detecting rumors from microblogs with recurrent neural networks",
abstract = "Microblogging platforms are an ideal place for spreading rumors and automatically debunking rumors is a crucial problem. To detect rumors, existing approaches have relied on hand-crafted features for employing machine learning algorithms that require daunting manual effort. Upon facing a dubious claim, people dispute its truthfulness by posting various cues over time, which generates long-distance dependencies of evidence. This paper presents a novel method that learns continuous representations of microblog events for identifying rumors. The proposed model is based on recurrent neural networks (RNN) for learning the hidden representations that capture the variation of contextual information of relevant posts over time. Experimental results on datasets from two real-world microblog platforms demonstrate that (1) the RNN method outperforms state-of-the-art rumor detection models that use hand-crafted features; (2) performance of the RNN-based algorithm is further improved via sophisticated recurrent units and extra hidden layers; (3) RNN-based method detects rumors more quickly and accurately than existing techniques, including the leading online rumor debunking services.",
author = "Jing Ma and Wei Gao and Prasenjit Mitra and Sejeong Kwon and Jansen, {Bernard J.} and Wong, {Kam Fai} and Meeyoung Cha",
year = "2016",
month = "1",
day = "1",
language = "English (US)",
volume = "2016-January",
pages = "3818--3824",
journal = "IJCAI International Joint Conference on Artificial Intelligence",
issn = "1045-0823",
}


@inproceedings{Yang2012AutomaticDO,
  title={Automatic detection of rumor on Sina Weibo},
  author={Fan Yang and Yang Liu and Xiaohui Yu and Min Yang},
  booktitle={MDS '12},
  year={2012}
}

@article{DBLP:journals/corr/abs-1904-13355,
  author    = {Kai Shu and
               Xinyi Zhou and
               Suhang Wang and
               Reza Zafarani and
               Huan Liu},
  title     = {The Role of User Profile for Fake News Detection},
  journal   = {CoRR},
  volume    = {abs/1904.13355},
  year      = {2019},
  url       = {http://arxiv.org/abs/1904.13355},
  archivePrefix = {arXiv},
  eprint    = {1904.13355},
  timestamp = {Thu, 02 May 2019 15:13:44 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1904-13355},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}


@inproceedings{Jin:2013:EMN:2501025.2501027,
 author = {Jin, Fang and Dougherty, Edward and Saraf, Parang and Cao, Yang and Ramakrishnan, Naren},
 title = {Epidemiological Modeling of News and Rumors on Twitter},
 booktitle = {Proceedings of the 7th Workshop on Social Network Mining and Analysis},
 series = {SNAKDD '13},
 year = {2013},
 isbn = {978-1-4503-2330-7},
 location = {Chicago, Illinois},
 pages = {8:1--8:9},
 articleno = {8},
 numpages = {9},
 url = {http://doi.acm.org/10.1145/2501025.2501027},
 doi = {10.1145/2501025.2501027},
 acmid = {2501027},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {SEIZ, SIS, epidemiological modeling, rumor detection},
} 

@inproceedings{Sampson:2016:LIS:2983323.2983697,
 author = {Sampson, Justin and Morstatter, Fred and Wu, Liang and Liu, Huan},
 title = {Leveraging the Implicit Structure Within Social Media for Emergent Rumor Detection},
 booktitle = {Proceedings of the 25th ACM International on Conference on Information and Knowledge Management},
 series = {CIKM '16},
 year = {2016},
 isbn = {978-1-4503-4073-1},
 location = {Indianapolis, Indiana, USA},
 pages = {2377--2382},
 numpages = {6},
 url = {http://doi.acm.org/10.1145/2983323.2983697},
 doi = {10.1145/2983323.2983697},
 acmid = {2983697},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {implicit network, rumor detection, social media},
} 


@inproceedings{ma-etal-2018-rumor,
    title = "Rumor Detection on Twitter with Tree-structured Recursive Neural Networks",
    author = "Ma, Jing  and
      Gao, Wei  and
      Wong, Kam-Fai",
    booktitle = "Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = jul,
    year = "2018",
    address = "Melbourne, Australia",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P18-1184",
    doi = "10.18653/v1/P18-1184",
    pages = "1980--1989",
    abstract = "Automatic rumor detection is technically very challenging. In this work, we try to learn discriminative features from tweets content by following their non-sequential propagation structure and generate more powerful representations for identifying different type of rumors. We propose two recursive neural models based on a bottom-up and a top-down tree-structured neural networks for rumor representation learning and classification, which naturally conform to the propagation layout of tweets. Results on two public Twitter datasets demonstrate that our recursive neural models 1) achieve much better performance than state-of-the-art approaches; 2) demonstrate superior capacity on detecting rumors at very early stage.",
}


@inproceedings{2c16b6ad1569495fac0bd5e212852b9d,
title = "Detect rumors in microblog posts using propagation structure via kernel learning",
abstract = "How fake news goes viral via social media? How does its propagation pattern differ from real stories? In this paper, we attempt to address the problem of identifying rumors, i.e., fake information, out of microblog posts based on their propagation structure. We firstly model microblog posts diffusion with propagation trees, which provide valuable clues on how an original message is transmitted and developed over time. We then propose a kernel-based method called Propagation Tree Kernel, which captures high-order patterns differentiating different types of rumors by evaluating the similarities between their propagation tree structures. Experimental results on two real-world datasets demonstrate that the proposed kernel-based approach can detect rumors more quickly and accurately than state-ofthe-art rumor detection models.",
author = "Jing Ma and Wei Gao and Wong, {Kam Fai}",
year = "2017",
month = "1",
day = "1",
doi = "10.18653/v1/P17-1066",
language = "English",
volume = "1",
pages = "708--717",
booktitle = "ACL 2017 - 55th Annual Meeting of the Association for Computational Linguistics, Proceedings of the Conference (Long Papers)",
publisher = "Association for Computational Linguistics (ACL)",
}


@paper{AAAI1816826,
	author = {Yang Liu and Yi-Fang Wu},
	title = {Early Detection of Fake News on Social Media Through Propagation Path Classification with Recurrent and Convolutional Networks},
	conference = {AAAI Conference on Artificial Intelligence},
	year = {2018},
	keywords = {fake news detection;social media;information propagation;recurrent and convolutional networks;deep learning},
	abstract = {In the midst of today's pervasive influence of social media, automatically detecting fake news is drawing significant attention from both the academic communities and the general public. Existing detection approaches rely on machine learning algorithms with a variety of news characteristics to detect fake news. However, such approaches have a major limitation on detecting fake news early, i.e., the information required for detecting fake news is often unavailable or inadequate at the early stage of news propagation. As a result, the accuracy of early detection of fake news is low. To address this limitation, in this paper, we propose a novel model for early detection of fake news on social media through classifying news propagation paths. We first model the propagation path of each news story as a multivariate time series in which each tuple is a numerical vector representing characteristics of a user who engaged in spreading the news. Then, we build a time series classifier that incorporates both recurrent and convolutional networks which capture the global and local variations of user characteristics along the propagation path respectively, to detect fake news. Experimental results on three real-world datasets demonstrate that our proposed model can detect fake news with accuracy 85% and 92% on Twitter and Sina Weibo respectively in 5 minutes after it starts to spread, which is significantly faster than state-of-the-art baselines.},

	url = {https://aaai.org/ocs/index.php/AAAI/AAAI18/paper/view/16826}
}


@inproceedings{Wang:2018:EEA:3219819.3219903,
 author = {Wang, Yaqing and Ma, Fenglong and Jin, Zhiwei and Yuan, Ye and Xun, Guangxu and Jha, Kishlay and Su, Lu and Gao, Jing},
 title = {EANN: Event Adversarial Neural Networks for Multi-Modal Fake News Detection},
 booktitle = {Proceedings of the 24th ACM SIGKDD International Conference on Knowledge Discovery \&\#38; Data Mining},
 series = {KDD '18},
 year = {2018},
 isbn = {978-1-4503-5552-0},
 location = {London, United Kingdom},
 pages = {849--857},
 numpages = {9},
 url = {http://doi.acm.org/10.1145/3219819.3219903},
 doi = {10.1145/3219819.3219903},
 acmid = {3219903},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {adversarial neural networks, deep learning, fake news detection},
} 


@article{DBLP:journals/corr/abs-1809-01286,
  author    = {Kai Shu and
               Deepak Mahudeswaran and
               Suhang Wang and
               Dongwon Lee and
               Huan Liu},
  title     = {FakeNewsNet: {A} Data Repository with News Content, Social Context
               and Dynamic Information for Studying Fake News on Social Media},
  journal   = {CoRR},
  volume    = {abs/1809.01286},
  year      = {2018},
  url       = {http://arxiv.org/abs/1809.01286},
  archivePrefix = {arXiv},
  eprint    = {1809.01286},
  timestamp = {Thu, 11 Oct 2018 15:59:45 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1809-01286},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
